On ML-Based Program Translation: Perils and Promises

With the advent of new and advanced programming languages, it becomes imperative to migrate legacy software to new programming languages. Unsupervised Machine Learning-based Program Translation could play an essential role in such migration, even without a sufficiently sizeable reliable corpus of parallel source code. However, these translators are far from perfect due to their statistical nature. This work investigates unsupervised program translators and where and why they fail. With in-depth error analysis of such failures, we have identified that the cases where such translators fail follow a few particular patterns. With this insight, we develop a rule-based program mutation engine, which pre-processes the input code if the input follows specific patterns and post-process the output if the output follows certain patterns. We show that our code processing tool, in conjunction with the program translator, can form a hybrid program translator and significantly improve the state-of-the-art. In the future, we envision an end-to-end program translation tool where programming domain knowledge can be embedded into an ML-based translation pipeline using pre- and post-processing steps.

==> body/2.definitions.tex <==
\section{Definitions}
\label{sec:definitions}
We will refer to the following wording throughout the rest of the paper. 

\noindent
\textit{Collapse.} A collapse is an example of which after translation of a code in either language, the output code does not contain the entirety of a function which resembles the original function that was translated. A collapse is also characterized by spam of certain characters or numbers. We refer to ‘import spam collapse’ as a collapse which, after a certain point, solely contains ‘import [x]’ over and over again. A screenshot is enclosed below in Figure [1]. We refer to ‘number spam collapse’ as a collapse which is characterized by strings of single digits, with commas in between. A screenshot is enclosed below in Figure [2]. We refer to ‘comma spam collapse’ as a collapse characterized by repetition of commas over one or more lines. A screenshot is enclosed below in Figure [3]. Finally, we refer to ‘spacetoken spam collapse’ as the repetition of SPACETOKEN at different points throughout one line of code. A screenshot is enclosed below in Figure [4]. 
% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=8cm]{figures/Figure1.png}
%     \caption{An example of import spam collapse}
% \end{figure}

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=8cm]{figures/Figure2.png}
%     \caption{An example of number spam collapse}
% \end{figure}

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=8cm]{figures/Figure3.png}
%     \caption{An example of comma spam collapse}
% \end{figure}

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=8cm]{figures/Figure4.png}
%     \caption{An example of spacetoken spam collapse}
% \end{figure}


% \begin{figure*}
%      \centering
%      \begin{subfigure}[b]{0.22\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/Figure1.png}
%          \caption{Import spam collapse}
%          \label{fig:collapse_import_spam}
%      \end{subfigure}
%      \hfill
%       \begin{subfigure}[b]{0.22\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/Figure2.png}
%          \caption{Number spam collapse}
%          \label{fig:collapse_num_spam}
%      \end{subfigure}
%      \hfill
%       \begin{subfigure}[b]{0.22\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/Figure3.png}
%          \caption{Comma spam collapse}
%          \label{fig:collapse_comma_spam}
%      \end{subfigure}
%      \hfill
%       \begin{subfigure}[b]{0.22\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/Figure4.png}
%          \caption{Spacetoken spam collapse}
%          \label{fig:collapse_spacetoken_spam}
%      \end{subfigure}
%         \caption{\small{\textbf{Examples of Collapse by Transcoder Model}}}
%         \label{fig:collapse}
% \end{figure*}

\begin{figure}[!ht]
    \centering
    \begin{minipage}{0.5\textwidth}
     \begin{lstlisting}[language=Python,]
def import ( ):
	import numpy , numpy , stream , numpy , array , numpy
	import numpy , tuple , tuple
	from numpy , tuple , tuple
	...
     \end{lstlisting}
    \end{minipage}

    \caption{An example of import spam collapse}
\end{figure}

\begin{figure}[!ht]
    \centering
    \begin{minipage}{0.5\textwidth}
     \begin{lstlisting}[language=Python,]
def test_count_minimum_subsequences_consecutive_NUMBERS ( ) :
	n_success = 0
	param0 = [ ]
	sample = [ 3 , 7, 11, 14 , 14 , 14 , 14 , 14, 14 , 14 , 14 , 14 ... ]
     \end{lstlisting}
    \end{minipage}
    \caption{An example of number spam collapse}
\end{figure}

\begin{figure}[!ht]
    \centering
    \begin{minipage}{0.5\textwidth}
     \begin{lstlisting}[language=Python,]
def ','','','','','','','','','','','','...
     \end{lstlisting}
    \end{minipage}
    \caption{An example of comma spam collapse}
\end{figure}

\begin{figure}[!ht]
    \centering
    \begin{minipage}{0.5\textwidth}
     \begin{lstlisting}[language=Python,]
def SPACETOKEN CEILING SPACETOKEN in SPACETOKEN a SPACETOKEN b SPACETOKEN c
     \end{lstlisting}
    \end{minipage}
    \caption{An example of spacetoken spam collapse}
\end{figure}

A complex for loop is a for loop that satisfies at least one of the following criteria: multiple conditions, multiple variables, or nonlinear variable modifications. An example of a complex for loop is shown in Figure [5]. 

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=8cm]{figures/Figure5.png}
%     \caption{An example of a complex for loop}
% \end{figure}

\begin{figure}[!ht]
    \centering
    \begin{minipage}{0.5\textwidth}
     \begin{lstlisting}[language=Java,]
for ( int x = curr ; x > 0 ;  x = x / 10 ) {
    sum = sum + x % 10 ;
}

     \end{lstlisting}
    \end{minipage}
    \caption{An example of a complex for loop}
\end{figure}




==> body/3.motivation.tex <==
\section{Motivation and Problem Formulation}
\label{sec:motivation}
Most modern programming language translators rely on supervised learning, which require large datasets of labelled translations. In this aspect, unsupervised learning is more efficient in the effort to translate between programming languages, generating these labelled datasets require tedious work. Facebook AI's \transcoder is the most popular model that accomplishes programming language translation using unsupervised learning fueled by a GeeksforGeeks unlabelled dataset. However, the accuracy of the model revealed in their paper, are less than optimal. Our work aims to discover the exact flaws of this model, and develop potential solutions to these weaknesses.

==> body/backup_5.result.tex <==
\label{sec:method}

\transcoder is the state-of-the-art and most popular model that accomplishes programming language translation using unsupervised learning fueled by a GeeksforGeeks unlabelled dataset. 
\transcoder is a gigantic transformer-based model consisting of 312 million parameters. Yet, their reported accuracy is still suboptimal: the computational accuracy of Python to Java translation is 68.7\%, and 56.1\% the other way around.

To understand what kind of errors \transcoder commonly makes, we dug deeper into the \transcoder-generated erroneous translations using 100 examples. 
Two of the authors went through the code examples, and noted their findings which were verified by another two authors. 
For each case, all of the authors reached a consensus about the type of potential error. 
To this end, we identify some common error patterns \transcoder is making. 
Leveraging these findings, we propose a hybrid technique combining machine learning and traditional template-based solutions that can give an end-to-end solution to the code translation problem. 


\subsection{Dataset} 
Facebook AI’s Github page ~\cite{facebookresearch} provided extensive testing data for the \transcoder model taken from the GeeksForGeeks dataset. The testing dataset provided is comprised of around 280 files each in Python, Java, and C++. Each file has a method, f\_gold(), which is to be translated, along with a main method containing test cases. Of roughly 850 given testing files in each language, we randomly sampled 50 test cases for both Java to Python and Python to Java translation analysis. For each test case, we ran the \transcoder to translate each file, analyzed the progress of each translation, marked what errors were similar in multiple file translations and potential solutions.




\subsection{Empirical Findings: Common Error Patterns}
\label{sec:results}

Based on this study, we identify 4 different categories of error.

\noindent
\textbf{1. Method Context.} The goal of the model is to accurately translate one method, typically called \textit{focal method}. However, the focal method is often surrounded by a \texttt{main} method and test cases. 
%which includes the function as well as the test cases that test the operation of said function. 
With such additional context, \transcoder tends to get confused between arguments inside and outside the method. 
Sometimes, the \transcoder opted to translate the associated test cases as well, resulting in incorrect or unreadable code.
Sometimes bogus code is appended with the intended translation. 
%that was incorrect, code that was correct but had unreadable code appended, or code that did not translate the function in question.
%seems to be unable to determine the difference between arguments inside and outside the function. In many of the tests we ran, TransCoder opted to translate the test cases as well, resulting in code that was incorrect, code that was correct but had unreadable code appended, or code that did not translate the function in question. 
9 out of 50 Java to Python (J2P) and 19 out of 50 Python to Java (P2J) examples suffer from this problem. 
%
%attempted a translation of the test cases. Contrary to our experience in Java to Python, the majority of these test cases resulted in a translation of the function with code appended to it. Two of those nineteen tests resulted in a collapse. After we removed the main method and once again attempted translation, this issue was seen to be resolved, as shown in Figure [7]. 
Once these focal methods are translated in isolation, \transcoder can generate the correct output. ~\Cref{eg:context} shows an example.
%attempted a translation of the test cases, thus resulting in code that was a translation of the main method with test cases, instead of f$\_$gold(). After we removed the main method and once again attempted translation, this issue was seen to be resolved, as shown in Figure [6]. 
	
% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=8cm]{figures/Figure6.png}
%     \caption{Main method removal removing number spam collapse in J2P}
% \end{figure}


% \begin{figure*}[!ht]
%     \centering
%     \begin{minipage}{0.3\textwidth}
%      \begin{lstlisting}[language=Java,caption=\small{Initial Java Code}]
% static int f_gold ( List<Integer> poly , int n , int x ) {
% 	int result = poly .get(0) ;
% 	for ( int i = 1 ;
% 	i < n ;
% 	i ++ ) result = result * x + poly .get(i) ;
% 	return result ;
% }
%      \end{lstlisting}
%     \end{minipage}
%     ~
%     \begin{minipage}{0.3\textwidth}
%      \begin{lstlisting}[language=Python, caption=\small{Initial Python Translation}]
% def test_horneRS_method_polynomisal_evaluation ( poly ,  n , x ) :
% 	n_success = 0
% 	param0 = [ ]
% 	sample = [ 3 , 18 , 22 , 27 , 31 , 33 , 36 ... ]
% 	param0.append ( sample )
% 	param1 = [-16 , 16 , 16 , 16 , 16 , 16 , 16 , ... ]

%      \end{lstlisting}
%     \end{minipage}
%    % ~
%    %  \begin{minipage}{0.3\textwidth}
%    %   \begin{lstlisting}[language=Java,caption= \small{Fixed Java Code: (Main Method Removal)}]
%    %      //Same Java code, but removed main method prior to translation
%    %   \end{lstlisting}
%    %  \end{minipage}
%     ~   
%     \begin{minipage}{0.3\textwidth}
%      \begin{lstlisting}[language=Python,caption=\small{Python translation after fixing}]
% def pyHORNERS_METHOD_POLYNOMIAL_EVALUATION ( poly , n , x ) :
% 	result = poly [ 0 ]
% 	for i in range ( 1 , n ) :
% 		result = result * x + poly [ i ]
% 	return result

%      \end{lstlisting}
%     \end{minipage}


%     \caption{\textbf{\small{Main method removal removing number spam collapse in J2P}}}
% \end{figure*}

% Nineteen of the fifty test cases from Python to Java attempted a translation of the test cases. Contrary to our experience in Java to Python, the majority of these test cases resulted in a translation of the function with code appended to it. Two of those nineteen tests resulted in a collapse. After we removed the main method and once again attempted translation, this issue was seen to be resolved, as shown in Figure [7]. 

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=8cm]{figures/Figure7.png}
%     \caption{Main method removal improving translation in P2J}
% \end{figure}


\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/Transpiler.drawio.pdf}
    \caption{\textbf{\small{Error Patterns and their proposed template-based solutions}}}
    \label{fig:error_patterns}
\end{figure*}


% \begin{figure*}[!ht]
%     \centering
%     \begin{minipage}{0.4\textwidth}
%      \begin{lstlisting}[language=Python,numbers=none,caption=\footnotesize{Initial Python Code}]
% def main():
%     ...
%     f_gold(...)
%     ...
       
% def f_gold ( mat , n ) :
% 	principal = 0 
% 	secondary = 0 ; 
% 	...
% 	print ( "Principal Diagonal:" , principal )
% 	print ( "Secondary Diagonal:" , secondary )
%      \end{lstlisting}
%     \end{minipage}
%     ~
%     \begin{minipage}{0.25\textwidth}
%      \begin{lstlisting}[language=Java,numbers=none,caption=\footnotesize{Initial Java Translation}]
%      // No translation, only tokenized function and nothing under it
%      \end{lstlisting}
%     \end{minipage}

%     Fixed Python Code [Main Method Removal]
%     \begin{minipage}{0.5\textwidth}
%      \begin{lstlisting}[language=Python,]
%      #Same Python code, but removed main method prior to translation
%      \end{lstlisting}
%     \end{minipage}

%     Initial Java Translation
%     \begin{minipage}{0.5\textwidth}
%      \begin{lstlisting}[language=Java,]
% public static void f_gold (int [ ] [ ]  mat , int n ) {
% 	int principal = 0 ;
% 	int secondary = 0 ;
% 	;
% 	...
% 	System . out . println ( "Principal Diagonal:" + principal ) ;
% 	System . out . println ( "Secondary Diagonal:" + secondary ) ;
% }
%      \end{lstlisting}
%     \end{minipage}
%     \caption{Main method removal improving translation in P2J}
%     \label{eg:context}
% \end{figure*}

% In both of these examples, resolved refers to that only the function was translated, but we do not make claims on the accuracy of these translations. Additionally, removing the main method effectively removes all occurrences of a number spam collapse, indicating that number spam collapses were due to the test cases of the main method. As demonstrated below, these translations still continue to have language specific issues that we will get into more detail about. 
	
		
In both Java to Python and Python to Java, we noted that even if there was no direct indication that the \transcoder was translating the main method, such as if the test cases appeared in the output file, the translation still benefited from removing the main method and only translating the function. 
One such example is below, of Java to Python, is shown in Figure [8].

\begin{figure}[!ht]
    \centering
    Initial Java Code
    \begin{minipage}{0.5\textwidth}
     \begin{lstlisting}[language=Java,]
static int f_gold ( List<Integer> arr, int n ) {
	int dp [ ] = new int [ n ] ; 
	...
	return result ;
}
     \end{lstlisting}
    \end{minipage}

    Initial Python Code [Collapse]
    \begin{minipage}{0.5\textwidth}
     \begin{lstlisting}[language=Python,]
def SPACETOKEN f ( param1 ) :
# return (param0).get(param1).get(param0).get(param0).get(param0)...
     \end{lstlisting}
    \end{minipage}

    Fixed Java Code [Main Method Removal]
    \begin{minipage}{0.5\textwidth}
     \begin{lstlisting}[language=Python,]
//Same Java code, but main method removed prior to translation
     \end{lstlisting}
    \end{minipage}
    
    Python Translation After Fixing
    \begin{minipage}{0.5\textwidth}
     \begin{lstlisting}[language=Java,]
def remMainMethod ( arr , n ) :
	dp = [ 1 for i in range ( n ) ]
	...
	return result
     \end{lstlisting}
    \end{minipage}

    \caption{Main method removal fixing spacetoken spam collapse in J2P}
\end{figure}

Translations after removing the main method also turned out to have slight differences, especially in the example of Python to Java. An example is demonstrated in Figure [9].

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=8cm]{figures/Figure9.png}
%     \caption{Main method removal improving translation in P2J}
% \end{figure}


\begin{figure}[!ht]
    \centering

Initial Python Code
\begin{minipage}{0.5\textwidth}
 \begin{lstlisting}[language=Python,]
 def f_gold ( A , B . n ) :
	sorted ( A )
	sorted ( B )
	result = 0
	for i in range ( n ) :
		result += ( A [ i ] + B [ n - i - 1 ] )
	return result

 \end{lstlisting}
\end{minipage}

Initial Java Translation
\begin{minipage}{0.5\textwidth}
 \begin{lstlisting}[language=Java,]
static int f_gold ( int [ ] A , int [ ] B , int n ) {
	Arrays . sort ( A ) ;
	Arrays . sort ( B ) ;
	int result  = 0 ;
	for ( int i = 0 ;
	i < n ;
	i ++ ) result += ( A [ i ]  * B [ n - i - 1 ] ) ;
	return result ;
}

 \end{lstlisting}
\end{minipage}

Fixed Python Code
\begin{minipage}{0.5\textwidth}
 \begin{lstlisting}[language=Python,]
#Same Python code, but removed main method prior to translation
 \end{lstlisting}
\end{minipage}

Java Translation After Fixing
\begin{minipage}{0.5\textwidth}
 \begin{lstlisting}[language=Java,]
public static double fGold ( double [ ] A , double [ ]  B, int n ) {
	Arrays . sort ( A ) ;
	Arrays . sort ( B ) ;
	double result = 0 ;
	for ( int i = 0 ;
	i < n ;
	i ++ ) {
		result += (A [ i ] * B [ n - i - 1 ] ) ;
	}
	return result ;
}

 \end{lstlisting}
\end{minipage}

    \caption{Main method removal improving translation in P2J}
\end{figure}

Therefore, for all of the shortcomings which we will discuss for the rest of the paper, we treat the TransCoder not as a purely code translator, but mainly as a function translator. The translation errors observed will henceforth be mainly errors that occurred when we singularly translated the functions using the TransCoder. 


\textit{\textbf{Java to Python Translation Analysis:}}

Within the Java to Python translations of the TransCoder model, the most prominent forms of collapse are importing spam collapse, spacetoken collapse, and comma spam collapse. Of the original 50 translated test cases from data collection, 28/50, or roughly half, of the test cases experienced some form of collapse during TransCoder translation.

By using preprocessing techniques, or modifying the files prior to translation, in a standardized manner, we were able to remove collapses from nearly all of the previously collapsed translations.

\textbf{Technique 1)} Translation of Complex For Loop to While Loop
As Java for loops generally allow for more complexities than Python for loops, the \transcoder model has difficulty translating complex for loops from Java to Python.

Complex for loops appeared in 6 test cases of the original 50 files, and all 6 of the test cases did not produce correct outputs, with 4 out of the 6 resulting in collapsed translations from the model.

We hypothesized it would be beneficial to convert these for loops to while loops before translation, while maintaining the same output, and determine if this change helps the translation. The following algorithm was developed to do this manual translation in a standardized manner: maintain the condition in the while loop, move the initialization to directly before while loop, and move variable updating to end of while loop, or directly before any breaks, continues, or return statements.

This change significantly improved the translation of all 6 of the test cases, and translation of several other hand-crafted complex for loops solidified the hypothesis that the model works better at translating while loops than for loops from Java to Python. This improvement is modeled in Figure [10].

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=8cm]{figures/Figure10.png}
%     \caption{Changing for loop to while loop fixing import spam collapse}
% \end{figure}

\begin{figure*}[!h]
\centering
%\begin{subfigure}[b]{0.45\textwidth}
\begin{minipage}{0.45\textwidth}
\centering
\begin{lstlisting}[language=Java, caption=\small{Initial Java Code}, numbers=none]
 static String f_gold ( List<Character> str , int len ) {
	int i = 0 , j = len - 1 ;
	for ( ; i < j ; i ++ , j -- ) {
		...
		System . out . println ( "Not Possible" ) ;
		return "" ; 
	}
	return String . valueOf ( str ) ;
}
\end{lstlisting} 
%\caption{\textbf{\small{Initial Java Code}}
\end{minipage}
%\end{subfigure}
~
\begin{minipage}{0.45\textwidth}
 \begin{lstlisting}[language=Python,caption=\small{Initial Python Translation},numbers=none]
def import ( ) :
	import inspect
	import inspect
	...
 \end{lstlisting}
\end{minipage}

\begin{minipage}{0.45\textwidth}
 \begin{lstlisting}[language=Java,caption=\small{Fixed Java Code (For to While)},numbers=none]
 static String f_gold ( List<Character> str , int len ) {
	int i = 0 , j = len - 1;
	while(i < j){
		...
		if ( str .get(i)== str .get(j) && str .get(i) != '*' ){
		    i++;
		    j--;
		    continue ;
		}
		...
		System . out . println ( "Not Possible" ) ;
		return "" ; 
	}
	return String . valueOf ( str ) ;
}
\end{lstlisting}
\end{minipage}
~
\begin{minipage}{0.45\textwidth}
 \begin{lstlisting}[language=Python,caption=\small{Python Translation After Fixing},numbers=none]
 def f_gold ( ) :
	i , j = 0, len
	while i < j :
		...
		if ( str .get(i)== str .get(j) && str .get(i) != '*' ):
		    i += 1
		    j -= 1
		    continue ;
		...
		print ( "Not Possible" )
		return ""
	return str
\end{lstlisting}
\end{minipage}
\caption{\textbf{\small{Changing for loop to while loop fixing import spam collapse}}}
\label{fig:loop}
\end{figure*}

\textbf{Technique 2)} Rewriting array parameters to Lists 
In a significant portion of the sampled test cases, 19 out of 50 test cases, f$\_$gold() contained a parameter that was some type of array. In every attempted translation of these test cases, there was some form of collapse within the model’s translation. The most common type of collapse that occurred was an importing spam collapse, specifically with the importing of numpy.

To modify f$\_$gold() prior to translation in a way that preserves the code’s meaning and output, but enables \transcoder to successfully translate it, we came up with the following algorithm: when there is an f$\_$gold() method that uses an array parameter, rewrite the parameter as a List of the wrapper class, and rewrite all methods of the original array to their respective List method.

By implementing this change of rewriting arrays to Lists, 15/19 of the test cases that previously collapsed had great improvement. The other 4/19 test cases had no improvement, but after removing the main method, we saw great improvement within them as well, as shown in Figure [11].

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=8cm]{figures/Figure12.png}
%     \caption{Changing array parameter to List fixing import spam collapse}
% \end{figure}


\begin{figure}[!ht]
    \centering

Initial Java Code
\begin{minipage}{0.5\textwidth}
 \begin{lstlisting}[language=Java,]
static int f_gold ( int arr [ ] , int n ) {
	HashMap < Integer , Integer > hmap = new HashMap < > ( ) ;
	...
	for ( Integer a : hmap . keySet ( ) ) {
		if ( hmap . get ( a) % 2 != 0 ) return a ;
	}
	return - 1 ;
}

 \end{lstlisting}
\end{minipage}

Initial Python Translate [Collapse]
\begin{minipage}{0.5\textwidth}
 \begin{lstlisting}[language=Python,]
 def import ( arr , n ) :
	import numpy , numpy , numpy , numpy ...

 \end{lstlisting}
\end{minipage}

Fixed Java Code [Array to List]
\begin{minipage}{0.5\textwidth}
 \begin{lstlisting}[language=Java,]
static int f_gold ( List<Integer> arr , int n ) {
	HashMap < Integer , Integer > hmap = new HashMap < > ( ) ;
	...
	for ( Integer a : hmap . keySet ( ) ) {
		if ( hmap . get ( a ) % 2 != 0 ) return a;
	}
	return -1 ;
}

 \end{lstlisting}
\end{minipage}

Python Translation After Fixing
\begin{minipage}{0.5\textwidth}
 \begin{lstlisting}[language=Python,]
 def find_the_number_occurrence_odd_number_of_times_1 ( arr , n ) :
	hmap = { }
	...
	for a in hmap.keys ( ) :
		if hmap [ a ] % 2 != 0 :
			return a
	return - 1

 \end{lstlisting}
\end{minipage}


    \caption{Changing array parameter to List fixing import spam collapse}
\end{figure}


\textit{\textbf{Python to Java Translation Analysis:}}



	In comparison to Java to Python translation, Python to Java suffered from much less collapse errors, and had an overall higher rate of success. As detailed above, the only two collapses that were observed occurred due to inclusion of the main method, which are all fixed by the removal of the aforementioned main method. The figures can be viewed above, in the section regarding removal of the main method. 

	The most prominent issue that plagues Python to Java translation lies within the addition of logical operators to if statements and else statements. Of the fifty test cases, twelve experienced the addition of logical operators to if statements which had the potential to either affect the code or not affect it at all. Below, we give examples of both. 
	
	The following is an example of when the addition of a logical operator will not affect the code in a significant manner. In the following examples, the conditions are repeated exactly with the ‘\&\&’ operator, meaning that the code will not be affected, as demonstrated within Figure [12].

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=8cm]{figures/Figure13.png}
%     \caption{Logical operator error}
% \end{figure}


\begin{figure}[!ht]
    \centering
Initial Python Code
\begin{minipage}{0.5\textwidth}
 \begin{lstlisting}[language=Python,]
 def f_gold ( n ) :
	res = 0
	x = 0
	while ( x * x < n ) :
		...
	return res

 \end{lstlisting}
\end{minipage}

Initial Java Translation [Added Logical Operator]
\begin{minipage}{0.5\textwidth}
 \begin{lstlisting}[language=Java,]
 public static int f_gold ( int n ) {
	int res = 0 ;
	int x = 0 ;
	while ( ( x * x < n ) && (x * x < n ) ) {
		...
	}
	return res ;
}

 \end{lstlisting}
\end{minipage}


    \caption{Logical operator error}
\end{figure}

The following is an example of when the addition of a logical operator will affect the code in a significant manner. In the following example, instead of merely asking that x not be equal to 0, we are also requested that x mod 10 is equal to 0, which is not necessary and puts extra conditions on the while loop itself, therefore barring the code from running like it was originally intended to. This is seen in Figure [13].

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=8cm]{figures/Figure14.png}
%     \caption{Logical operator error}
% \end{figure}

\begin{figure}[!ht]
    \centering
    
Initial Python Code
\begin{minipage}{0.5\textwidth}
 \begin{lstlisting}[language=Python,]
 def f_gold ( x ) :
	temp = x
	n = 0
	while ( x != 0 ) :
		...
	return ( sm == temp )

 \end{lstlisting}
\end{minipage}

Initial Java Translation [Added Logical Operator]
\begin{minipage}{0.5\textwidth}
 \begin{lstlisting}[language=Java,]
 static final public int f_gold ( int x ) {
	int temp = x ;
	int n = 0 ;
	while ( ( x != 0 ) && ( x % 10 == 0 ) ) {
		...
	return ( sm == temp ) ? 1 : 0 ;
}

 \end{lstlisting}
\end{minipage}


    \caption{Logical operator error}
\end{figure}

Note that in all of these examples, the extra logical operators append an entirely new condition and do not change or affect the old condition in of itself, which is translated correctly. Therefore, we are able to manually take out any conditions following the original one which we do not want. In our examples, we also found that one condition is appended to each statement, usually. Therefore, if we had n conditions in our if statement or while loop, there would be n+1 conditions in the Java translation. 

The other issue we observed within Python to Java translation involved preprocessing very similar to Java to Python translation issues. Upon the existence of two or more arrays with ‘arr’ as parameters in the python code, our code experienced collapse. There were two test cases that satisfied these conditions, and both of them collapsed. However, it may be of interest to note that when only one array ‘arr’ was used, there was no such issue, as seen in Figure [14].
	
	
% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=8cm]{figures/Figure15.png}
%     \caption{Array naming solution fixing number spam collapse}
% \end{figure}

\begin{figure}[!ht]
    \centering

Initial Python Code
\begin{minipage}{0.5\textwidth}
 \begin{lstlisting}[language=Python,]
def f_gold ( arr1, arr2 , m , n , k ) :
    sorted1 = [ 0 ] * ( m + n )
	...
	return sorted1 [ k - 1]

 \end{lstlisting}
\end{minipage}

Initial Java Translation [Collapse]
\begin{minipage}{0.5\textwidth}
 \begin{lstlisting}[language=Java,]
  - 1 , 0 , 0 , 0 , 0 , 0 , 0 , 0 , 0 ...

 \end{lstlisting}
\end{minipage}

Fixed Python Code [arr to list]
\begin{minipage}{0.5\textwidth}
 \begin{lstlisting}[language=Python,]
 
def f_gold ( list1, list2 , m , n , k ) :
    sorted1 = [ 0 ] * ( m + n )
	...
	return sorted1 [ k - 1]

 \end{lstlisting}
\end{minipage}

Java Translation After Fixing
\begin{minipage}{0.5\textwidth}
 \begin{lstlisting}[language=Java,]
 public static int f_gold ( int [ ] list1 , int [ ] list2 , int m , int n , int k ) {
	int [ ] sorted1 = new int [ m + n ] ;
	...
	return sorted1 [ k - 1] ;
}
 \end{lstlisting}
\end{minipage}


    \caption{Array naming solution fixing number spam collapse}
\end{figure}

The manual fix for this is easy. As lists and arrays in python are the same, all we needed to do was every occurrence of ‘arr’ with ‘list’. This rendered our code able to be translated by the \transcoder model. 

